Middleware for LLMs: Tools Are Instrumental for Language Agents in Complex Environments

The applications of large language models (LLMs) have expanded well beyond the confines of text processing, signaling a new era where LLMs are envisioned as generalist agents capable of operating within complex environments. These environments are often highly expansive, making it impossible for the LLM to process them within its short-term memory. Motivated by recent research on extending the capabilities of LLMs with tools, we seek to investigate the intriguing potential of tools to augment LLMs in handling such complexity by introducing a novel class of tools, termed middleware, to aid in the proactive exploration within these massive environments. Such specialized tools can serve as a middleware layer shielding the LLM from environmental complexity. In two representative complex environments -- knowledge bases (KBs) and databases -- we demonstrate the significant potential of augmenting language agents with tools in complex environments. Notably, equipped with the middleware, GPT-4 achieves 2.8X the performance of the best baseline in tasks requiring access to database content and 2.2X in KB tasks. Our findings illuminate the path for advancing language agents in real-world applications.

==> acknowledgements.tex <==
\section*{Acknowledgements}
We would like to thank colleagues from the OSU NLP group and THU KEG for their thoughtful comments.
In addition, we are grateful to the authors of \Bird for kindly providing the original predictions of the baselines based on API Docs prompting. 
This research was supported by Cisco Research.
